QuickCSG: Fast Arbitrary Boolean Combinations of N Solids

QuickCSG computes the result for general N-polyhedron boolean expressions without an intermediate tree of solids. We propose a vertex-centric view of the problem, which simplifies the identification of final geometric contributions, and facilitates its spatial decomposition. The problem is then cast in a single KD-tree exploration, geared toward the result by early pruning of any region of space not contributing to the final surface. We assume strong regularity properties on the input meshes and that they are in general position. This simplifying assumption, in combination with our vertex-centric approach, improves the speed of the approach. Complemented with a task-stealing parallelization, the algorithm achieves breakthrough performance, one to two orders of magnitude speedups with respect to state-of-the-art CPU algorithms, on boolean operations over two to dozens of polyhedra. The algorithm also outperforms GPU implementations with approximate discretizations, while producing an output without redundant facets. Despite the restrictive assumptions on the input, we show the usefulness of QuickCSG for applications with large CSG problems and strong temporal constraints, e.g. modeling for 3D printers, reconstruction from visual hulls and collision detection.

==> complexity.tex <==


\section{Performance and Theoretical Complexity}
%
Discussion of complexity of 2-poly CSG previously analyzed. Reference to relevant papers.

\subsection{Asymptotic Lower Bound}
%
Provide analysis for each algorithm stage and conclude over dominant asymptotic phase.

\subsection{Optimality}
Justification.

%
%
%

\newcommand{\Nf}{N_\mathrm{f}}
\newcommand{\Ninleaf}{N_\mathrm{inleaf}}
\newcommand{\Csplit}{C_\mathrm{split}}
\newcommand{\ccheck}{C_\mathrm{check}}

\matthijsS{
To do a rough complexity computation, we assume:
\begin{itemize}
\item
  the KDTree is a balanced binary tree,
\item
  facets that are not split. This is close to true for meshes with compact facets like toruses,
\item 
  it is fully constructed, without  pruning the tree,
\item
  the splitting stops when there are less than $\Ninleaf$ facets in a node. This parameter is important to balance the cost of building the tree vs. the cost of the search.
\end{itemize}

In this case, the tree is of depth $\log_2 (\Nf / \Ninleaf)$ with $\Nf
/ \Ninleaf$ leaves. Noting the cost of splitting a node with $m$
facets as $\Csplit m$, the cost of building the tree is
\begin{equation}
 \Nf \Csplit \log_2 \frac{\Nf}{\Ninleaf}
\end{equation}

Function~\textsc{CSGVertices} is applied locally on each leaf, which costs:
\begin{equation}
\frac{\Nf}{\Ninleaf} \Ninleaf^3 \ccheck
\end{equation}
Therefore, the total cost is: 
\begin{equation}
C_\mathrm{kdtree} = \Nf \Csplit \log_2 \frac{\Nf}{\Ninleaf} +  \Nf \Ninleaf^2 \ccheck
\end{equation}

}


==> related.tex <==
\section{Related Work}
\label{sec:relatedwork}
%
(grey area here as to what part should go here and be mentionned in intro)

general considerations over state of the art, milestones.

polyhedral intersection largely studied and giving rise to well known subproblems: robustness and exact arithmetic, optimiztion of algorithm. The evolution and milestones might be the subject of the introduction as well...

the problem is considered largely solved and has subsequently been much less active in the last decade, aside from specific improvements and optimizations

\subsection{Genesis of the two-polyhedron CSG algorithm}

\begin{itemize}
\item polyhedron data-structures, cone intersections: Baumgart
\item 80's algorithmic generalization and robustness considerations: Hoffmann 89
\item 90's: exact computations ( Fortune, ...), non piecewise linear geometry (BOOLE, todo refs...): 
\end{itemize}

Conclusion: no algorithm looking at the problem other than with poly-to-poly view. The N-polyhedral case never (?) specifically addressed.

\subsection{Robustness}

Exact Arithmetic Computations, Symbolic perturbations, CGAL Nef polyhedra...

conclusion: we follow paper on approximate perturbations yet our algorithm could be applied for exact algorithms.

\subsection{Hierarchical representations}

\begin{itemize}
\item -tree introduction for polyhedral representation (lookup ref, 80's)
\item BSP trees / Naylor: Merging BSP trees, Segura 2013
\end{itemize}

conclusion: Hierachical representation concern the geometry of a single polyhedron. Performance not improved as much as if the kd-tree is built to embed the whole problem to specifically build it for CSG optimization as proposed.

\subsection{Specific Optimizations}

\begin{itemize}
\item CPU optimizations, multithread: Dinesh Manosha's Boole system.
\item GPU-based parallel optimizations: Depth-Layered Image 
\end{itemize}

Cite EPVH somewhere here?

Say somewhere -- since our algorithm is vertex-centric, it does not require to follow edges, which requires complicated synchronization points when multithreading [MenierParallelEPVH].



Still two poly centered. DLI is an approximation.
Interesting stuff existing on ray-shooting with kd-trees: all the SAH stuff.

\subsection{Notable Implementations}

Boole, CGAL, GTS, Carve CSG. What else?


